Unsupervised Multi-Modal Image Registration via Geometry Preserving Image-to-Image Translation

Many applications, such as autonomous driving, heavily rely on multi-modal data where spatial alignment between the modalities is required. Most multi-modal registration methods struggle computing the spatial correspondence between the images using prevalent cross-modality similarity measures. In this work, we bypass the difficulties of developing cross-modality similarity measures, by training an image-to-image translation network on the two input modalities. This learned translation allows training the registration network using simple and reliable mono-modality metrics. We perform multi-modal registration using two networks - a spatial transformation network and a translation network. We show that by encouraging our translation network to be geometry preserving, we manage to train an accurate spatial transformation network. Compared to state-of-the-art multi-modal methods our presented method is unsupervised, requiring no pairs of aligned modalities for training, and can be adapted to any pair of modalities. We evaluate our method quantitatively and qualitatively on commercial datasets, showing that it performs well on several modalities and achieves accurate alignment.

==> figures/Cross-metric/fig.tex <==
\begin{figure}
    \centering
    \includegraphics[width=.4\textwidth]{figures/Cross-metric/cross-modality-metric.jpg}
    \caption{zzzz: \dc{this is a placeholder.. we need a nice example with two closeup insets.}}
    \label{fig:cross-metric}
\end{figure}

==> figures/bilateral_numerical/fig.tex <==
\begin{table}
    \centering
    \begin{center}
        \begin{tabular}{||l c c||} 
        \hline
        Method & Test Acc. &  Train Acc. \\ [0.5ex] 
        \hline\hline
        No Registration & 35.45  & 34.96 \\
        \hline
        W/O Bilateral   &  11.01 & 9.89 \\
        \hline
        With Bilateral   &  6.93 & 6.12 \\
        \hline
        \end{tabular}
    \end{center}
    \caption{Smoothness Regularization - Effect of bilateral filtering on registration accuracy.}
    \label{fig:bilateral_numerical}
\end{table}




==> figures/deformation_field_network/fig.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{figures/deformation_field_network/Network.pdf}
    \caption{Deformation Field Network. \moab{Under construction... any ideas for improvement are welcomed.}}
    \label{fig:training_overview}
\end{figure}
